Deep electric field predictions by drift-reduced Braginskii theory with plasma-neutral interactions based upon experimental images of boundary turbulence

We present 2-dimensional turbulent electric field calculations via physics-informed deep learning consistent with (i) drift-reduced Braginskii theory under the framework of an axisymmetric fusion plasma with purely toroidal field and (ii) experimental estimates of the fluctuating electron density and temperature on open field lines obtained from analysis of gas puff imaging of a discharge on the Alcator C-Mod tokamak. The inclusion of effects from the locally puffed atomic helium on particle and energy sources within the reduced plasma turbulence model are found to strengthen correlations between the electric field and electron pressure. The neutrals are also directly associated with broadening the distribution of turbulent field amplitudes and increasing ${\bf E \times B}$ shearing rates. This demonstrates a novel approach in plasma experiments by solving for nonlinear dynamics consistent with partial differential equations and data without encoding explicit boundary nor initial conditions.

==> table-comments.tex <==
\begin{tabular}{ |p{1.5cm}||p{1.5cm}|p{2.0cm}|p{2.5cm}|p{2.5cm}|p{2.5cm}| }
 \hline
 \multicolumn{6}{|c|}{PINN diagnostics ($n_e, T_e$)} \\
 \hline
 JobID & $N_f = N_0$ & L-BFGS $\#$ & $\mathcal{L}_2$ ($n_e$) &$\mathcal{L}_2$ ($T_e$) &$\mathcal{L}_2$ ($E_r$)\\
 \hline
 30592030 & 1     & 569734  & 0.007024932    & 0.058694724 & 0.006954913
\\
 30592040 & 5     & 410369  & 0.025779343    & 0.302535922 & 0.006954913
\\
 30592032 & 10    & 468396  & 0.022521256    & 0.222615523 & 22130014784
\\
 30592033 & 50    & 232208  & 0.000118963    & 0.114065990 & 0.006954913
\\
 30592034 & 100   & 251260  & 0.000043194    & 0.001635210 & 0.006954913
\\
 30592035 & 500   & 468706  & 0.000020832    & 0.000191519 & 0.001144108
\\
 30592036 & 1000  & 332982  & 0.000027763    & 0.000071774 & 0.000655993
\\
 30592037 & 5000  & 85232   & 0.000098833    & 0.000270884 & 0.006955764
\\
 30592038 & 10000 & 32476   & 0.000136675    & 0.000340698 & 0.003472795
\\
 \hline
\end{tabular}

Attached is an example table relevant to the results in the paper that I could include if sought, but I think still better suited to the longer manuscript. There are a few nuances for why this table looks different from Raissi et al, and I'll simply note these details below if you're interested but, substantially, they're not all too important and different versions/modifications can be easily made:

I have set $N_f$ (number of random mini-batch points for learning observed 2-dimensional measurements of $n_e$ and $T_e$ in each iteration) = $N_0$ (number of random mini-batch collocation points for evaluating the PDE in each iteration). These two quantities certainly do not have to be equal. Additionally, one may even argue that $N_0$ should be 0 until observed measurements (i.e. $n_e$ and $T_e$) are learned (e.g. errors in columns 4 and 5 should be lower than $10^{-4}$ before making $N_0 != 0$), but this assumes perfect measurements, and would not be a wise choice if data is noisy. Nevertheless, this is the simplest choice for producing a table and is not explicitly a challenge for the scenarios Raissi et al tackle as it is here in inferring unknown in a multi-field model.

All runs are defined to only run for 20 hours. Therefore, I have set column 3 as a proxy for the number of iterations based upon the number of cumulative iterations taken by the L-BFGS optimizer when training against the model simply as a diagnostic. Just noting that there is also the Adam optimizer in these examples. Additionally, there are further iterations beyond just training on the model, e.g. when training on the observed data of $n_e$ and $T_e$. Comparing cases with just L-BFGS or just Adam and with further modifications to these optimizers (e.g. different parameters, adaptive weights) could be other interesting comparisons. But that is for another paper...

Perhaps the only quantity that matters is the last column, the average L2-norm error of the radial electric field when evaluating all points in the 2-dimensional space of the Letter's figures. I include the average L2-norm for $n_e$ and $T_e$ to note it is still being learned by the PINN and affected by the choice of $N_f$.

I can also include the L2-norm for $f_{n_e}$ and $f_{T_e}$. I simply prefer to look at the L2-norm of $E_r$ instead since the former can hit a local minimum (e.g. a trivial solution to the PDE) and be very low despite not actually being very accurate.

In this particular table, I have provided all data and am performing mini-batch sampling with the batch sample size given by $N_0$ and $N_f$. It is also possible to not provide all data but instead only a fraction. But once again, this is simply one of many possible changes one can perform (depending upon the experimental scenario of interest) and will warrant other changes to improve the algorithm depending on the sparseness of data.

Result: number of optimizer iterations decreases with $N_0$, but does not necessarily mean accuracy is good. The important figure of merit is L2-norm for Er (even beyond $f_1$ and $f_5$). which indicates whether learning by the PINNs is going well, and yes, for 20 hours of training, choosing approximately $N_0 = N_f = 500 - 1000$ is optimal, but other approaches such as training first on data and then the model may yield even better results depending upon noise in observed measurements.
